Out-of-Distribution Detection and Selective Generation for Conditional Language Models

Machine learning algorithms typically assume independent and identically distributed samples in training and at test time. Much work has shown that high-performing ML classifiers can degrade significantly and provide overly-confident, wrong classification predictions, particularly for out-of-distribution (OOD) inputs. Conditional language models (CLMs) are predominantly trained to classify the next token in an output sequence, and may suffer even worse degradation on OOD inputs as the prediction is done auto-regressively over many steps. Furthermore, the space of potential low-quality outputs is larger as arbitrary text can be generated and it is important to know when to trust the generated output. We present a highly accurate and lightweight OOD detection method for CLMs, and demonstrate its effectiveness on abstractive summarization and translation. We also show how our method can be used under the common and realistic setting of distribution shift for selective generation (analogous to selective prediction for classification) of high-quality outputs, while automatically abstaining from low-quality ones, enabling safer deployment of generative language models.

==> TODO.tex <==
\textcolor{red}{
\section{TODOs}
\begin{itemize}
% \item Add quality by dataset for summarization, rouge-1 and human eval
%\item Ensure Figure text is readable.
%\item Fix intro
% \item add definition for perplexity (we already have it in section 2)
% \item add an algorithm
%\item Edit and trim
%\item ensure ROUGE, BLEURT use macros for consistency
%\item standardize percentile sum abbreviation
%\item standardize ML -> Linear reg.
\end{itemize}
}

==> old/MT.tex <==
\section{Expriments for Translation}
\label{exp_trans}
\todo{merge into respective sections alongside summarization}

\toaddjl{overview/segway goes here.}

\subsection{Experimental Setup}

Moved to \ref{sec:exp_detection}

\subsection{Results}

% \textcolor{blue}{One paragraph to explain the law dataset.}
% We additionally note that all methods fail to distinguish \texttt{law} from \texttt{holdout}. 
% Through analysis of $n$-gram overlap between the various test sets and the training data, 
% we observe that \texttt{law} has the 
% highest unigram overlap rate (48.8\%) and the second highest overall overlap after \texttt{holdout} (\Figref{fig:ngram}).\footnote{We define overlap rate as the percentage of unique $n$-grams in the test set that are also present in the training data. 
% The overall overlap is defined as the geometric mean of all the $n$-gram overlap rates up to $n=4$.
% All domains/splits including the training data are subsampled to 1K for this analysis.}
% This suggests that \texttt{law} is actually close to the in-domain distribution, and as a result, all methods fail
% to adequately differentiate between \texttt{law} and \texttt{holdout}.


% \include{tex/figure_translation_ngram_overlap}

% \begin{table}[]
% \begin{tabular}{lllllllll}
%                             & \multicolumn{3}{l}{Near shift OOD}                      & \multicolumn{5}{l}{Far shift OOD}           \\
% measure                     & newstest2014 & newsdiscussdev2015 & newsdiscusstest2015 & law   & medical & koran & IT    & subtitles \\
% \multicolumn{9}{l}{Input OOD}                                                                                                       \\
% GPT-3 likelihood (baseline) & TBD          & TBD                & TBD                 & TBD   & TBD     & TBD   & TBD   & TBD       \\
% Maha (baseline)             & 0.544        & 0.641              & 0.629               & 0.512 & 0.635   & 0.732 & 0.702 & 0.822     \\
% Relative Maha (ours)        & 0.790        & 0.843              & 0.834               & 0.337 & 0.845   & 0.949 & 0.942 & 0.955     \\
% Binary logits (ours)        & 0.847        & 0.885              & 0.879               & 0.471 & 0.808   & 0.953 & 0.895 & 0.938     \\
% \multicolumn{9}{l}{Output OOD}                                                                                                      \\
% Perplexity (baseline)       & 0.578        & 0.587              & 0.574               & 0.394 & 0.415   & 0.726 & 0.432 & 0.489     \\
% COMET (baseline)            & 0.526        & 0.622              & 0.592               & 0.419 & 0.600   & 0.728 & 0.715 & 0.676     \\
% Prism (baseline)            & 0.422        & 0.504              & 0.490               & 0.477 & 0.588   & 0.729 & 0.606 & 0.557     \\
% Maha (baseline)             & 0.607        & 0.723              & 0.741               & 0.473 & 0.773   & 0.833 & 0.902 & 0.932     \\
% Relative Maha (ours)        & 0.781        & 0.833              & 0.822               & 0.318 & 0.833   & 0.927 & 0.934 & 0.940     \\
% Binary logits (ours)        & 0.813        & 0.845              & 0.850               & 0.489 & 0.786   & 0.931 & 0.876 & 0.904    
% \end{tabular}
% \end{table}



==> old/defs.tex <==
% % \newcommand{\y}{Y}
% \newcommand{\x}{\mathbf{x}}
% \newcommand{\z}{\mathbf{z}}
% \newcommand{\mdist}{\text{MDist}}
% \newcommand{\rmdist}{\text{RMDist}}
% \newcommand{\gaussx}{\mathcal{N}(\mathbf{\vmu}^{\vz}, \vSigma^{\vz})}
% \newcommand{\gaussy}{\mathcal{N}(\mathbf{\vmu}^{\vw}, \vSigma^{\vw})}
% \newcommand{\gaussxo}{\mathcal{N}(\mathbf{\vmu}^{\vz}_0, \vSigma^{\vz}_0)}
% \newcommand{\gaussyo}{\mathcal{N}(\mathbf{\vmu}^{\vw}_0, \vSigma^{\vw}_0)}
% \newcommand{\gaussk}{\mathcal{N}(\mathbf{\vmu}_k, \vSigma)}
% \newcommand{\gausso}{\mathcal{N}(\mathbf{\vmu}_0,\vSigma)}
% \newcommand{\C}{\mathcal{C}}
% \newcommand{\U}{\mathcal{U}}


% %%%%% NEW MATH DEFINITIONS %%%%%

% \usepackage{amsmath,amsfonts,bm}

% % newer macros
% \newcommand{\D}{\mathcal{D}}
% \newcommand{\Y}{\mathcal{Y}}
% \newcommand{\Reals}{\mathbb{R}}
% %\newcommand{\vTheta}{{\bm{\Theta}}}
% \newcommand{\ytilde}{\tilde{y}}
% \newcommand{\vxtilde}{\tilde{\vx}}
% \newcommand{\data}{\{\vx_n, y_n\}_{n=1}^N}
% \newcommand{\map}{\mathsf{MAP}}
% \newcommand{\wmap}{\mathsf{WMAP}}
% \newcommand{\dataset}{{\cal D}}
% \newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}




% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% % \newcommand{\train}{\mathcal{D}}
% % \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% % \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}
% \def\vmu{{\bm{\mu}}}
% \def\vSigma{{\bm{\Sigma}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% % Don't use a set called E, because this would be the same as our symbol
% % for expectation.
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak


==> old/section_ood_method_20220924.tex <==
\section{OOD Detection in Conditional Language Generation Models}

\subsection{Perplexity is not a good OOD detector}
\label{sec:perplexity_for_ood}

Maximum softmax probability (MSP) $p(\hat{y}|\vx)$, $\hat{y}=\argmax_{k=1,\dots,K} p(y=k|\vx)$ was the most basic and commonly used OOD score for the $K$-class classification problem \citep{hendrycks2016baseline,lakshminarayanan2017simple}. For a conditional language generation model, the output is a sequence of predicted tokens $\{\hat{y}_0 \hat{y}_1 \dots, \hat{y}_L\}$, and each has a conditional softmax probability $p(\hat{y}^{t}|\hat{y}^{<t}, \vx)$, $\hat{y}^{t}=\argmax_{v\in V} p(y^{t}=v|\hat{y}^{<t}, \vx)$, $t=1,\dots,L$ and $V$ is the token vocabulary. The perplexity score, which is the average negative log-probability over tokens in the sequence $-\frac{1}{L} \sum_{t=1}^{L} \log p(\hat{y}^{t}|\hat{y}^{<t}, \vx)$, can be regarded as a natural extension of the the MSP score for OOD detection in conditional generative models. 

We first study how well the perplexity score performs for OOD detection tasks, using summarization and translation as two different tasks. 
% Perplexity score is not well suited for OOD detection. 
In Figure \ref{fig:ppx_hist}, we compare the distribution of perplexity score of (a) a summarization model and (b) a translation model trained on in-domain dataset and evaluated on multiple OOD datasets, respectively.
For summarization, a model is trained on \texttt{xsum} (BBC news) and evaluated on test splits of other news datasets including \texttt{cnn\_dailymail} and \texttt{newsroom} as near-OOD datasets, and forum (\texttt{forumsum}) and dialogue (\texttt{samsum} and \texttt{reddit\_tifu}) datasets as far-OOD. 
The perplexity distribution have quite overlap with each other even though the input format are significantly different. Furthermore, perplexity assigns \texttt{cnn\_dailymail} even lower scores than the in-domain \texttt{xsum}. 

For translation, the model is trained on WMT15 dataset and evaluated on other WMT test splits \cite{bojar-etal-2015-findings} and OPUS100 \cite{tiedemann-2012-parallel}. The in-domain and OOD datasets have the similar distribution under perplexity, largely overlapping to each other.
Overall, both experiments show that perplexity is not suited for OOD detection. 

% \todo{prism}



\begin{figure}[!htb]
\centering
\begin{subfigure}[t]{0.45\textwidth} % changed for arxiv
\centering
\caption{Summarization}
% \vspace{-0.1em}
\includegraphics[width=\textwidth]{figures/hist_perplexity_with_legend.pdf} 
\end{subfigure} 
% \vspace{-0.8em}
\begin{subfigure}[t]{0.45\textwidth} % changed for arxiv
\centering
\caption{Translation}
% \vspace{-0.1em}
\includegraphics[width=\textwidth]{figures/translation/hist_perplexity_with_legend.pdf}
\end{subfigure} 
% \vspace{-0.1em}
% \vspace{-0.8em}
% \begin{subfigure}[t]{0.30\textwidth} % changed for arxiv
%     \centering
%     \caption{Correlation (ppx, rouge1) decreases as OOD increases}
%     % \vspace{-0.1em}
%     \includegraphics[width=0.95\textwidth]{figures/corr_ppx_decrease_as_ood_increase.pdf}
%     \label{fig:train_vs_auc}
% \end{subfigure} 
\caption{
Histograms of perplexity scores of a generation model trained on a single domain (\xsum for summarization, and WMT for translation) and evaluated on multiple other domains.
% Perplexity score is not suited for OOD detection. For summarization, perplexity assigns cnn\_dailymail even lower scores than in-domain xsum, which is not expected. For translation, in-domain and OOD datasets have the similar distribution under perplexity, largely overlapping to each other.
}
\label{fig:ppx_hist}
\end{figure}




\subsection{Proposed method: Embedding based lightweight OOD detector}
\label{sec:ood_detection_proposed_method}

We developed a lightweight OOD detection method based on text embeddings. 
Our method does not require re-training of the generation model or deploying a separate scoring models, and the computation cost of our OOD scores is negligible because the text embeddings are derived readily from the generative model itself. 

Text embeddings, especially those from pre-trained models, have been shown to provide rich semantic representation, and enable many successful downstream natural language inference tasks \citep{devlin2018bert,aharoni2020unsupervised}. We propose to use the input and output embeddings to detect OOD as shown in Figure \ref{fig:diagram}. 

In this work, we use Transformer encoder-decoders for conditional language generation and the \textbf{input embedding} is obtained from the encoder by averaging the encoder's final-layer hidden state vectors corresponding to the input sequence tokens. To obtain the \textbf{output embedding}, we first generate/decode conditioned on the input then average the decoder final-layer hidden state vectors corresponding to the decoded tokens.

Intuitively, if the text embedding of the test input or output is far from the embedding distribution of the training data, the test input is more likely to be OOD. 

\begin{figure}[!htb]
\centering
\includegraphics[width=0.6\textwidth]{figures/text_OOD_diagram_v1.pdf}
\caption{The proposed OOD detector based on input and output embeddings. 
}
% (b) The proposed combined quality score based on OOD scores and Perplexity that predicts output quality (rouge, bleu, huamn eval etc.) better than individual scores. \todo{Put figures next to each other?}
\label{fig:diagram}
\end{figure}

Mahalanobis distance (Maha) \citep{lee2018simple} is a widely used OOD detection method based on embeddings for classification models. It fits $K$ class-conditional Gaussian distributions for the corresponding $K$ in-distribution classes, based on the embeddings of the training data belonging to that class. At inference time, it measures the distance between the test input to the fitted Gaussian. 

Unlike the classification models that have  class labels, in the text encoder-decoder models, we have a paired input and output text sequences. 
We propose to fit one Gaussian distribution for input $\gaussx$ and a second Gaussian distribution for output $\gaussy$, using the training data. 
In particular, for an input and output text pair ($\vx$, $\vy$), we denote $\vz=f(\vx)$ as the input embedding, and $\vw=g(\vy)$ as the output embedding. 
Given the training data $(\vx_i, \vy_i)$ and their corresponding embeddings $(\vz_i,\vw_i), i=1\dots N$, the mean and covariance matrix are estimated as 
% $\mathbf{\vmu}^{(\cdot)} = \frac{1}{N} \sum_{i=1}^N \vz^{(\cdot)}_i$,
%   and $\vSigma^{(\cdot)} = \frac{1}{N}\sum_{i=1}^N ( \vz^{(\cdot)}_i-\mathbf{\vmu}^{(\cdot)})(\vz_i^{(\cdot)}-\mathbf{\vmu}^{(\cdot)})^T$, where $(\cdot) \in \{\vx, \vy$\}.
$\mathbf{\vmu}^{\vz} = \frac{1}{N} \sum_{i=1}^N \vz_i$,
and $\vSigma^{\vz} = \frac{1}{N}\sum_{i=1}^N ( \vz_i-\mathbf{\vmu}^{\vz})(\vz_i-\mathbf{\vmu})^T$. 
Similarly $\mathbf{\vmu}^{\vw}$ and $\vSigma^{\vw}$ are estimated accordingly using $\vw_i$.
For a test input and output embedding pair $(\vz_{\text{test}}, \vw_{\text{test}})$, the input Maha distance is computed as 
\begin{align*}
\text{MD}({\vz_{\text{test}}}) = \left(\vz_{\text{test}}-\mathbf{\vmu}^{\vz}\right)^T (\vSigma^{\vz})^{-1} \left(\vz_{\text{test}}-\mathbf{\vmu}^{\vz} \right). \tag{\footnotesize Input Maha OOD score}
\end{align*}
The output Maha distance $\text{MD}({\vw_{\text{test}}})$ is computed similarly using $\vw_{\text{test}}$ based on $\gaussy$,
\begin{align*}
\text{MD}({\vw_{\text{test}}}) = \left(\vw_{\text{test}}-\mathbf{\vmu}^{\vw}\right)^T (\vSigma^{\vw})^{-1} \left(\vw_{\text{test}}-\mathbf{\vmu}^{\vw} \right). \tag{\footnotesize Output Maha OOD score}
\end{align*}

Mahalanobis distance is equivalent to computing a negative log-likelihood of the Gaussian distribution (up to a constant and a scalar), i.e. $-\log p(\vz)=\frac{d}{2}\log(2\pi)+\frac{1}{2}\log|\vSigma|+\frac{1}{2}(\vz-\vmu)^T \vSigma^{-1}(\vz-\vmu) = \texttt{const.} + \frac{1}{2} \text{MD}(\vz)$. It is known that the likelihood score derived from the deep neural networks can be easily confounded by background features in images and genomics \citep{ren2019likelihood}. 
We found it is also true in text. Mahalanobis distance is highly affected by the proportion of stop words in the text (for example, the correlation between input Maha distance and proportion of stop words is -0.21, suggesting a text with few stop words will has a high Maha score, regardless if it is from OOD our in-domian).

\paragraph{Relative Mahalanobis distance for OOD detection} 
To remove the stop words effect and other background confounding factors, inspired by \cite{ren2019likelihood}, we propose Relative Mahalanobis distance (Relative Maha, RMD), which is the relative difference between the original Maha distance to a baseline Maha distance. Specifically, 
\begin{align}
\text{RMD}({\vz_{\text{test}}}) \nonumber = \text{MD}({\vz_{\text{test}}}) - \text{MD}_0({\vz_{\text{test}}}), \tag{\footnotesize Input RMD OOD score}
% \label{eq:ratio}
\end{align}
where $\text{MD}_0({\vz_{\text{test}}})=\left(\vz_{\text{test}}-\mathbf{\vmu}^{\vz}_0\right)^T (\vSigma^{\vz}_0)^{-1} \left(\vz_{\text{test}}-\mathbf{\vmu}^{\vz}_0 \right)$ is the baseline Maha distance to a fitted background Gaussian distribution $\gaussxo$. The background distribution is supposed to be fitted using a large and broad dataset to represent the distribution of all variety of domains. 
The samples in the background dataset are fed into the corresponding conditional language model to obtain the input and output embeddings, and the embeddings are then used to fit an input background Gaussian $\gaussxo$, and an output background Gaussian $\gaussyo$ respectively. 
Similar to the input RMD score, the output RMD score is,
\begin{align}
\text{RMD}({\vw_{\text{test}}}) \nonumber = \text{MD}({\vw_{\text{test}}}) - \text{MD}_0({\vw_{\text{test}}}), \tag{\footnotesize Output RMD OOD score}
% \label{eq:ratio}
\end{align}
where $\text{MD}_0({\vw_{\text{test}}})=\left(\vw_{\text{test}}-\mathbf{\vmu}^{\vw}_0\right)^T (\vSigma^{\vz}_0)^{-1} \left(\vw_{\text{test}}-\mathbf{\vmu}^{\vw}_0 \right)$ is the Maha distance to the fitted background distribution $\gaussyo$.

In practice, we use \texttt{C4}, a colossal, cleaned version of the Common Crawl’s web crawl corpus \footnote{\url{https://www.tensorflow.org/datasets/catalog/c4}} and \texttt{para\_crawl/enfr} dataset, the web-scale parallel corpora for translation \footnote{\url{https://www.tensorflow.org/datasets/catalog/para_crawl}}, as the data for fitting background model for summarization and translation respectively. 
The RMD score can be regarded as a background contrastive score that indicates how close the test example to the training domain compared with that to the general domain.
A negative score suggests the examples is from in-domain, while a positive score suggests the example is from OOD. The higher the score indicates the greater the OOD-ness. Zero (0) can be a natural threshold for OOD detection. 

\paragraph{Binary classifier for OOD detection}
Another natural model for distinguishing the in-domain from a general domain is a binary classification model trained on in-domain data and the background data. Based on the input/ output embeddings of the two training sets (in-domain training data as the negative set, paired with the same number of general domain training data as the positive set), we train a simple logistic regression model with intercept and weight coefficient parameters $(\beta_0, \bm{\beta_1})$. As for the OOD score, we propose to use the un-normalized logits, 
\begin{align*}
\text{Binary logits}(\vz_{\text{test}}) = \beta_0 + \bm{\beta_1} \vz_{\text{test}}. \tag{\footnotesize Input Binary logits OOD score}
% \text{Binary logits}(\vw_{\text{test}}) = \beta_0 + \bm{\beta_1} \vw_{\text{test}}. \tag{\footnotesize Output Binary logits OOD score}
\end{align*}
The higher logits score suggests higher likelihood of OOD. The preferred use of the logits over of probability was also recommended by previous OOD studies for classification problems \citep{hendrycks2019scaling}.  
Similarly we propose the output binary logits OOD score as,
\begin{align*}
\text{Binary logits}(\vw_{\text{test}}) = \gamma_0 + \bm{\gamma_1} \vw_{\text{test}}. \tag{\footnotesize Output Binary logits OOD score}
\end{align*}

\paragraph{The connection between RMD and Binary classifier}
RMD is a generative model based approach which assumes the distributions of the two classes are Gaussian, while the binary classifier is a discriminative model which learns the decision boundary between two classes. 
Though they have different settings, under certain condition, the two Gaussian generative model can be reduced to a binary classifier.  
To see the connection, let us assume the label $y=0$ if the sample is from in-domain, and $y=1$ if the sample is from the general domain. Let us also assume the two classes have balanced sample size without loss of generality $p(y=1)=p(y=0)$. 
Since the log-probability of $\log p(y=1|\vz)$ can be rewritten using the Bayes rule $\log p(y=1|\vz) = \log p(\vz|y=1) + \log p(y=1) - \log p(\vz)$, the logit (log odds) can be written as,
\begin{align*}
\text{logit} = \log \left(\frac{p(y=1|\vz)}{p(y=0|\vz)} \right) &= \log p(y=1|\vz) - \log p(y=0|\vz) \\
&= \log p(\vz|y=1) - \log p(\vz|y=0) \\
&= -\frac{1}{2} \left(\text{MD}_{(\vmu_{y=1}, \vSigma_{y=1})}(\vz) - \text{MD}_{(\vmu_{y=0}, , \vSigma_{y=0})}(\vz) \right) + \texttt{const.}
% &= -\frac{1}{2} [ \left(\log|\vSigma_{y=1}|-\log|\vSigma_{y=0}|\right) - \left((\vz-\vmu_{y=1})^T \vSigma_{y=1}^{-1}(\vz-\vmu_{y=1}) - (\vz-\vmu_{y=0})^T \vSigma_{y=0}^{-1}(\vz-\vmu_{y=0}) \right) ]
\end{align*}
When $\vSigma = \vSigma_{y=1}=\vSigma_{y=0}$, the equation can be further simplified as 
\begin{align*}
\text{logit} &= \vSigma^{-1}(\vmu_{y=1}-\vmu_{y=0})^T\vz - \frac{1}{2} \left( \vmu_{y=1}^T \vSigma^{-1} \vmu_{y=1} - \vmu_{y=0}^T \vSigma^{-1} \vmu_{y=0} \right) + \texttt{const.} \\
&= \bm{\beta_1} \vz + \beta_0.
\end{align*}
Therefore, when assuming the covariance matrix are the same in two distributions, the two Gaussian  model is reduced to a binary classification model. 
However, our RMD does not assume the same covariance matrix in both distribution. We estimate the covariance matrix individually for each class. So our RMD is different from binary classifier, and it has higher model capacity than the binary classifier. 


\todo{add an algorithm}


==> old/table_ood_detection_sum.tex <==

\begin{table}[h]
% \begin{tabular}{llll}
%                  & \multicolumn{3}{l}{far-OOD}      \\
% measure          & reddit\_tifu & forumsum & samsum \\
% Input OOD        &              &          &        \\
% Maha             & 0.980        & 0.981    & 0.996  \\
% Relative Maha    & 0.998        & 0.998    & 0.999  \\
% Binary probs     & 0.999        & 0.999    & 0.994  \\
% GPT-3 likelihood &              &          &        \\
% Output OOD       &              &          &        \\
% Maha             & 0.987        & 0.975    & 0.986  \\
% Relative Maha    & 0.998        & 0.995    & 0.997  \\
% Binary probs     & 0.995        & 0.994    & 0.993  \\
% Perplexity       & 0.915        & 0.801    & 0.853 
% \end{tabular}
\small
\begin{tabular}{ccccccc}
                 & \multicolumn{2}{c}{Near Shift OOD}       & \multicolumn{3}{c}{Far Shift OOD}      \\
Measure          & \texttt{cnn\_dailymail} & \texttt{newsroom} & \texttt{reddit\_tifu} & \texttt{forumsum} & \texttt{samsum} \\ \toprule
\multicolumn{6}{c}{Input OOD}                                        \\ 
GPT-3 likelihood (baseline) &   TBD     &    TBD    &        TBD      &     TBD     &   TBD  \\   
Maha (baseline)           & 0.651          & 0.799         & 0.974        & 0.977    & 0.995 \\
Relative Maha (ours)   & 0.828          & 0.930         & 0.998        & 0.997    & 0.999  \\
Binary logits (ours)    & 0.997          & 0.959         & 1.000        & 0.999    & 0.998  \\ \midrule
\multicolumn{6}{c}{Output OOD}   \\ 
Perplexity (baseline)      & 0.424          & 0.665         & 0.909        & 0.800    & 0.851  \\
NLI score (baseline)           & 0.440          & 0.469         & 0.709        & 0.638    & 0.743 \\ 
Maha (baseline)            & 0.944          & 0.933         & 0.985        & 0.973    & 0.985  \\
Relative Maha (ours)   & 0.958          & 0.962         & 0.998        & 0.993    & 0.998  \\
Binary logits (ours)     & 0.989          & 0.982         & 1.000        & 0.998    & 0.997  \\ \bottomrule
\end{tabular}
\caption{AUROCs for far-OOD detection between \texttt{xsum} (in-domain) and the shifted OOD datasets. \texttt{cnn\_dailymail} and \texttt{newsroom} are considered as near shift OOD since it shares news topics as \texttt{xsum}, and \texttt{reddit\_tifu}, \texttt{forumsum}, and \texttt{samsum} are far shift OOD. All methods except for perplexity and NLI score have good OOD detection performance with AUROC $>0.95$ for far-OOD datasets. Among them, relative Mahalanobis distance and binary classifier perform the best and have similar AUROC values. For near shift OOD \texttt{cnn\_dailymail} and \texttt{newsroom}, binary classifier has the highest AUROCs $0.997$ for input and $0.985$ for output.}
%, as high as or even higher than the AUROC for far-OOD, suggesting binary classifier score is over-confident such that it loses the resolution for distinguishing near-OOD vs far-OOD.
\label{table:detection_aucroc_sum}
\end{table}


==> old/table_ood_detection_translate.tex <==
\begin{table}[h]
    \small
    \begin{tabular}{lcccccccc}
        \toprule
                              & \mc{3}{c}{WMT}  & \mc{5}{c}{OPUS}               \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-9} 
        Measure               & \texttt{nt2014} & \texttt{ndd2015} & \texttt{ndt2015} & \texttt{law} & \texttt{medical} & \texttt{Koran} & \texttt{IT} & \texttt{sub} \\ 
        \midrule\midrule
        \mc{9}{c}{\textsc{Input OOD}} \vspace{0.5em} \\
        Maha       & 0.534           & 0.671            & 0.670            & 0.511        & 0.704            & 0.737          & 0.828       & 0.900              \\
        Relative Maha  & 0.798           & 0.866            & 0.863            & 0.389        & 0.840            & 0.957          & 0.959       & 0.969              \\
        Binary logits  & 0.864           & 0.904            & 0.904            & 0.485        & 0.813            & 0.963          & 0.928       & 0.950              \\ 
        \midrule\midrule
        \mc{9}{c}{\textsc{Output OOD}} \vspace{0.5em} \\
        Perplexity & 0.570           & 0.496            & 0.494            & 0.392        & 0.363            & 0.657          & 0.343       & 0.359              \\
        COMET      & 0.484           & 0.514            & 0.525            & 0.435        & 0.543            & 0.632          & 0.619       & 0.518              \\
        Prism     & 0.445           & 0.504            & 0.505            & 0.459        & 0.565            & 0.716          & 0.604       & 0.577              \\
        Maha       & 0.609           & 0.733            & 0.739            & 0.482        & 0.784            & 0.838          & 0.900       & 0.935              \\
        Relative Maha  & 0.786           & 0.858            & 0.861            & 0.355        & 0.845            & 0.939          & 0.951       & 0.959              \\
        Binary logits & 0.822           & 0.860            & 0.865            & 0.507        & 0.783            & 0.942          & 0.890       & 0.910              \\ \bottomrule
    \end{tabular}
    \caption{\toaddjl{AUCROCs for translation OOD detection}}
    \label{table:detection_aucroc_translate}
\end{table}

==> old/table_quality_by_dataset_MT.tex <==
\begin{table}[h]
\caption{Translation quality for different MT datasets (higher is better). All datasets are sub-sampled to 1000 sentence pairs.}
\center
\begin{tabular}{lrr}
\toprule
dataset          & \texttt{BLEURT} & \texttt{BLEU} \\ 
\midrule
\texttt{law}     & 0.781                      & 53.8                     \\
\texttt{nt2014}  & 0.731                      & 39.8                     \\ 
\texttt{holdout} & 0.674                      & 41.8                     \\
\texttt{ndt2015} & 0.671                      & 37.9                     \\
\texttt{ndd2015} & 0.664                      & 30.9                     \\
\texttt{medical} & 0.643                      & 34.2                     \\
\texttt{IT}      & 0.588                      & 28.3                     \\
\texttt{sub}     & 0.552                      & 22.8                     \\
\texttt{Koran}   & 0.491                      & 12.9                     \\
\bottomrule
\end{tabular}
\label{tab:quality_by_dataset_MT}
\end{table}


==> old/table_quality_by_dataset_sum.tex <==
\begin{table}[]
\caption{Summarization quality (higher is better) for \xsum model. \rougeone is based on all samples in the test split per dataset, while human evaluation is based on 100.
The raw human evaluation rating was from 1-5. We normalized the score by dividing 5.0, and toke the median of the ratings over 3 raters. }
\center
\begin{tabular}{lrr}
\toprule
dataset          & \rougeone & Human evaluation \\ 
\midrule
\texttt{xsum}     &    0.474        &     0.698                 \\
\texttt{cnn\_dailymail}     &      0.226   &    0.624                  \\
\texttt{reddit\_tifu}     &      0.140 & 0.450                      \\
\texttt{samsum}     &      0.210   &           0.376           \\
\bottomrule
\end{tabular}
\label{tab:quality_by_dataset_sum}
\end{table}

==> old/table_quality_correlation_combined.tex <==
% consider putting this in appendix.
\begin{table}[h]
\begin{subtable}[c]{1\textwidth}
\centering
\subcaption{Summarization}
\scriptsize
\begin{tabular}{lccccc}
\toprule
                 & \multicolumn{1}{c}{In-domain} & \multicolumn{1}{c}{Near Shift OOD}       & \multicolumn{2}{c}{Far Shift OOD}      \\
Measure         &  \texttt{xsum} & \texttt{cnn\_dailymail} & \texttt{reddit\_tifu} & \texttt{samsum} & All datasets \\ \toprule
\multicolumn{6}{c}{Single Score} \\ \midrule    
% \multicolumn{6}{c}{Input OOD}  \\
% Maha (baseline)                                         & 0.044(5.6E-01)  & -0.018(8.1E-01) & -0.017(8.2E-01) & 0.133(8.3E-02) & 0.328(4.5E-19) \\
% Binary Logits (ours)                              & -0.022(7.7E-01) & -0.061(4.1E-01) & 0.028(7.1E-01)  & 0.106(1.7E-01) & 0.233(2.2E-10) \\
% \multicolumn{6}{c}{Output OOD}                                                                                                       \\
% \rowcolor{Gray}
Perplexity (baseline)                                 & 0.256  & 0.186  & \textcolor{gray}{0.081}  & \textcolor{gray}{0.068} & 0.300 \\
Nli score (baseline)                                   & 0.337  & 0.308  & 0.226  & \textcolor{gray}{0.132} & 0.381 \\
% Maha (baseline)                                  & 0.106(1.6E-01)  & -0.055(4.6E-01) & 0.202(7.2E-03)  & 0.352(4.7E-06) & 0.384(1.8E-25) \\
Input Relative Maha                                & \textcolor{gray}{0.015}  & \textcolor{gray}{-0.033} & \textcolor{gray}{0.017}  & \textcolor{gray}{0.133} & 0.336 \\
% \rowcolor{Gray}
Output Relative Maha                                 & \textcolor{gray}{0.053}  & 0.177  & 0.214  & 0.314 & 0.385 \\
% Binary Logits (ours)                        & 0.199(8.3E-03)  & -0.100(1.8E-01) & 0.091(2.3E-01)  & 0.026(7.4E-01) & 0.213(7.6E-09) \\
\multicolumn{6}{c}{Combined Score}  \\ \midrule
pct comb (ppx, input RMD)                    & 0.186  & \textcolor{gray}{0.134}  & \textcolor{gray}{0.082}  & \textcolor{gray}{0.109} & 0.358 \\
pct comb (ppx, output RMD)                   & \textcolor{gray}{0.250}  & 0.350  & 0.168  & 0.237 & \underline{0.415} \\
% pct comb (ppx, input binary logits)          & 0.214(5.1E-03)  & 0.079(2.9E-01)  & 0.126(1.0E-01)  & 0.090(2.4E-01) & 0.322(3.3E-18) \\
% pct comb (ppx, output binary logits)         & 0.347(6.6E-06)  & 0.086(2.5E-01)  & 0.114(1.3E-01)  & 0.052(5.0E-01) & 0.330(5.0E-19) \\
% pct sum (ppx, input \& output RMD)           & 0.171(2.6E-02)  & 0.242(1.3E-03)  & 0.158(3.7E-02)  & 0.250(1.3E-03) & 0.401(2.3E-27) \\
% pct sum (ppx, input \& output binary logits) & 0.277(3.4E-04)  & 0.003(9.7E-01)  & 0.127(9.5E-02)  & 0.096(2.2E-01) & 0.307(1.1E-16) \\
ML (ppx, input \& output)                                       & 0.235  & 0.402  & 0.170  & 0.250 & \textbf{0.422} \\ \bottomrule
\end{tabular}
\vspace{2em}
\end{subtable}
\begin{subtable}[c]{1\textwidth}
\centering
\subcaption{Translation}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
& \mc{4}{c}{WMT} & \mc{5}{c}{OPUS} & \\
\cmidrule(lr){2-5} \cmidrule(lr){6-10}
\multirow{-2}{*}{Measure} & \texttt{holdout} & \texttt{nt2014} & \texttt{ndd2015} & \texttt{ndt2015} & \texttt{law} & \texttt{medical} & \texttt{Koran} & \texttt{IT} & \texttt{sub} & \multirow{-2}{*}{All datasets} \\
\midrule
\mc{11}{c}{Single Score} \\
\midrule
% \mc{11}{c}{\textsc{Input OOD}} \vspace{0.5em} \\
% Maha & \llap{-}0.081 & \llap{-}0.131 & \llap{-}0.129 & \llap{-}0.117 & \llap{-}0.171 & \textcolor{gray}{0.041} & \llap{-}0.147 & \llap{-}0.093 & \textcolor{gray}{0.012} & 0.017 \\
% Binary logits & 0.144 & 0.116 & 0.141 & 0.162 & 0.124 & \textcolor{gray}{\llap{-}0.003} & \textcolor{gray}{0.025} & \llap{-}0.071 & 0.104 & 0.193 \\
% \midrule
% \mc{11}{c}{\textsc{Output OOD}} \vspace{0.5em} \\
% \rowcolor{Gray}
Perplexity & 0.309 & 0.337 & 0.352 & 0.375 & 0.389 & 0.224 & 0.222 & 0.225 & 0.227 & 0.274 \\
COMET & 0.184 & 0.397 & 0.402 & 0.443 & 0.324 & 0.253 & 0.359 & 0.174 & 0.297 & 0.320 \\
Prism & 0.184 & 0.329 & 0.337 & 0.342 & 0.179 & 0.188 & 0.192 & 0.151 & 0.286 & 0.286 \\
% Maha & \textcolor{gray}{\llap{-}0.029} & \llap{-}0.066 & \llap{-}0.064 & \llap{-}0.048 & \llap{-}0.096 & \textcolor{gray}{0.032} & \llap{-}0.105 & \llap{-}0.057 & \textcolor{gray}{0.041} & 0.086 \\
Input Relative Maha & 0.147 & 0.091 & 0.049 & 0.115 & 0.197 & \textcolor{gray}{0.013} & \llap{-}0.071 & \llap{-}0.060 & 0.098 & 0.191 \\
Output Relative Maha & 0.086 & 0.049 & 0.044 & 0.095 & 0.135 & \textcolor{gray}{\llap{-}0.026} & \llap{-}0.077 & \llap{-}0.056 & 0.061 & 0.167 \\
% Binary logits & 0.106 & 0.058 & 0.075 & 0.114 & 0.094 & \textcolor{gray}{\llap{-}0.036} & \textcolor{gray}{\llap{-}0.013} & \llap{-}0.059 & \textcolor{gray}{\llap{-}0.012} & 0.148 \\
\midrule
\mc{11}{c}{Combined Score} \\
\midrule
pct sum(ppx, input RMD) & 0.321 & 0.361 & 0.351 & 0.410 & 0.382 & 0.230 & 0.161 & 0.154 & 0.261 & \textbf{0.354} \\
pct sum(ppx, output RMD) & 0.323 & 0.357 & 0.359 & 0.414 & 0.371 & 0.200 & 0.152 & 0.164 & 0.240 & \underline{0.349} \\
% pct sum(ppx, input binary logits) & 0.323 & 0.352 & 0.372 & 0.384 & 0.391 & 0.195 & 0.211 & 0.111 & 0.234 & 0.326 \\
% pct sum(ppx, output binary logits) & 0.318 & 0.302 & 0.314 & 0.350 & 0.356 & 0.168 & 0.162 & 0.127 & 0.156 & 0.293 \\
% pct sum(ppx, input \& output RMD) & 0.291 & 0.284 & 0.264 & 0.329 & 0.346 & 0.119 & 0.082 & 0.084 & 0.231 & 0.305 \\
% pct sum(ppx, input \& output binary logits) & 0.300 & 0.262 & 0.288 & 0.309 & 0.340 & 0.125 & 0.145 & 0.053 & 0.163 & 0.281 \\
ML(ppx, input \& output) & 0.318 & 0.370 & 0.355 & 0.414 & 0.383 & 0.243 & 0.180 & 0.119 & 0.268 & 0.343 \\ \bottomrule
\end{tabular}
}
\end{subtable}
\caption{Kendall’s tau correlation (p-value $<0.05$ are grayed out) between various measures and human-judged quality score for summarization and \texttt{BLEURT} for translation. The "All datasets" column shows the correlation when all dataset examples are merged.}
\label{tab:quality_corr_combine}
\end{table}

==> tex/figure_translation_quality.tex <==

\begin{figure}[!htb]
    \centering
    %  \begin{subfigure}[t]{0.45\textwidth} % changed for arxiv
    %     \centering
    %     \caption{\toaddjl{caption}}
    %     % \vspace{-0.1em}
    %     \includegraphics[width=0.9\textwidth]{figures/translation/corr_ppx_bleurt_by_ood_input.png}
    % \end{subfigure} 
    % \vspace{0.8em}
    \begin{subfigure}[t]{0.30\textwidth} % changed for arxiv
        \centering
        \caption{\toaddjl{caption}}
        % \vspace{-0.1em}
        \includegraphics[width=0.9\textwidth]{figures/translation/cm_MT.png}
    \end{subfigure} 
    % \vspace{-0.1em}
    % \vspace{-0.8em}
    \begin{subfigure}[t]{0.30\textwidth} % changed for arxiv
        \centering
        \caption{Abstention Rate vs Quality \bleurt) Curve}
        % \vspace{-0.1em}
        \includegraphics[width=0.9\textwidth]{figures/translation/abstain_vs_quality.pdf}
    \end{subfigure} 
    \vspace{0.8em}
    \begin{subfigure}[t]{0.30\textwidth} % changed for arxiv
        \centering
        \caption{Survivorship per Dataset}
        % \vspace{-0.1em}
        \includegraphics[width=0.9\textwidth]{figures/translation/survivorship_line.png}
    \end{subfigure} 
    % \vspace{-0.1em}
    % \vspace{-0.8em}
    \caption{\toaddjl{caption}}
    \label{fig:translation_quality}
\end{figure}
